Reap the Harvest on Blockchain: A Survey of Yield Farming Protocols

Yield farming represents an immensely popular asset management activity in decentralized finance (DeFi). It involves supplying, borrowing, or staking crypto assets to earn an income in forms of transaction fees, interest, or participation rewards at different DeFi marketplaces. In this systematic survey, we present yield farming protocols as an aggregation-layer constituent of the wider DeFi ecosystem that interact with primitive-layer protocols such as decentralized exchanges (DEXs) and protocols for loanable funds (PLFs). We examine the yield farming mechanism by first studying the operations encoded in the yield farming smart contracts, and then performing stylized, parameterized simulations on various yield farming strategies. We conduct a thorough literature review on related work, and establish a framework for yield farming protocols that takes into account pool structure, accepted token types, and implemented strategies. Using our framework, we characterize major yield aggregators in the market including Yearn Finance, Beefy, and Badger DAO. Moreover, we discuss anecdotal attacks against yield aggregators and generalize a number of risks associated with yield farming.

==> exhibits/algo_lending.tex <==
\begin{algorithm}[tbp]
  \small
  \floatname{algorithm}{Strategy}
  \caption{Simple lending}
  \label{algo:simple_lending}
  \begin{algorithmic}[1]
    \STATE {\bf Deposit} assets in a lending protocol.
    \STATE {\bf Accrue} supply interest and {\bf collect} native tokens over time.
    \STATE {\bf Withdraw} deposits with accrued supply interest.
  \end{algorithmic}
\end{algorithm}

==> exhibits/algo_leveraged.tex <==
\begin{algorithm}[tbp]
  \small
  \floatname{algorithm}{Strategy}
  \caption{Leveraged lending}
  \label{algo:leveraged_borrow}
  \begin{algorithmic}[1]
    \STATE {\bf Deposit} assets in a lending protocol
    \STATE {\bf Borrow} assets with the deposits as collateral. \label{state:borrow}
    \STATE {\bf Deposit} borrowed assets. \label{state:redeposit}
    \STATE {\bf Repeat} steps \ref{state:borrow}--\ref{state:redeposit} multiple times.
    \STATE {\bf Accrue} interest and {\bf collect} native tokens over time.
    \STATE {\bf Swap} the native tokens into the assets borrowed.
    \STATE {\bf Repay} loans with accrued borrow interest.
    \STATE {\bf Withdraw} deposits with accrued supply interest when needed.
  \end{algorithmic}
\end{algorithm}

==> exhibits/algo_lp.tex <==
\begin{algorithm}[bp]
  \small
  \floatname{algorithm}{Strategy}
  \caption{Liquidity provision}
  \label{algo:liquidity_provision}
  \begin{algorithmic}[1]
    \STATE {\bf Provide} assets as liquidity in an AMM pool.
    \STATE {\bf Collect} native tokens over time.
    \STATE {\bf Withdraw} liquidity.
  \end{algorithmic}
\end{algorithm}

==> exhibits/comparison_table.tex <==
% \setlength{\tabcolsep}{5pt}
\begin{table*}[htbp]
% \footnotesize
\setlength{\tabcolsep}{4pt}
\caption{Overview of major existing yield aggregators}
\begin{tabularx}{\linewidth}{@{}X@{\hspace{1pt}}llllllllrlrrr@{}}
\toprule

& & \multicolumn{3}{c}{\ref{item:phase0}} & \multicolumn{3}{c}{\ref{item:phase2}} & & & & & & \\
& & \multicolumn{3}{c}{Supported pool assets} & \multicolumn{3}{c}{Strategies} & & & & & & \\
            \cmidrule(lr){3-5} \cmidrule(lr){6-8} 

\textbf{Protocol} &
& \textbf{Single} & \textbf{LP} & \textbf{Multiple} & \textbf{Simple} & \textbf{Leveraged} & \textbf{Liquidity} & \textbf{Pool} & \textbf{\# of} & \textbf{Governance} & \textbf{MCap*} & \textbf{TVL} & \textbf{Token}\\
%\textbf{FDV}

& & \textbf{asset} & \textbf{token} & \textbf{assets} & \textbf{lending} & \textbf{borrow} & \textbf{provision} & \textbf{name} & \textbf{pools} & \textbf{token} & \textbf{(m USd)} & \textbf{(m USd)} & \textbf{holders}\\

\midrule

Idle Finance & \cite{idle2021} & \CIRCLE & \Circle & \Circle & \CIRCLE & \Circle & \Circle & Pool & 10 & \tokenaddress{IDLE}{0x875773784Af8135eA0ef43b5a374AaD105c5D39e} & 29.8 & 105.8 & 3,704\\
Pickle Finance & \cite{pickle2021} & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \CIRCLE & pJar & 19 & \tokenaddress{PICKLE}{0x429881672B9AE42b8EbA0E26cD9C73711b891Ca5} & 9.2 & 88.5 & 7,238\\
Harvest Finance & \cite{harvest2021} & \CIRCLE & \CIRCLE & \Circle & \CIRCLE & \Circle & \CIRCLE & Vault & 53 & \tokenaddress{FARM}{0xa0246c9032bC3A600820415aE600c6388619A14D} & 64.3 & 295.5 & 12,003\\
Yearn Vaults & \cite{yearn2021} & \CIRCLE & \CIRCLE & \Circle &  \CIRCLE & \CIRCLE & \CIRCLE & Vault & 50 & \tokenaddress{YFI}{0x0bc529c00C6401aEF6D220BE8C6Ea1667F6Ad93e} & 1,156.6 & 5,548.1 & 44,484\\
Vesper & \cite{vesper2021} & \CIRCLE & \Circle & \Circle & \CIRCLE & \Circle & \Circle & Grow Pool & 4 & \tokenaddress{VSP}{0x1b40183efb4dd766f11bda7a7c3ad8982e998421} & 286.4 & 927.3 & 9,458\\
% Alpha Homora & \cite{alpha2021home} & & & & & & & & &  & & \\
Rari Capital Earn & \cite{rari2021}  & \CIRCLE & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle &  Pool & 3 & \tokenaddress{RGT}{0xD291E7a03283640FDc51b121aC401383A46cC623} & 157.5 & 196.9 & 9,559\\
Value DeFi & \cite{valuedefi2021} & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \CIRCLE & vSafe & 4 & \tokenaddress{VALUE}{0x49E833337ECe7aFE375e44F4E3e8481029218E5c} & 36.2 & 959.5 & 4,928 \\
\bottomrule
\end{tabularx}
\scriptsize \vskip 1mm
Data fetched in December 2021.

In \ref{item:phase0}, some farming pools only accept single assets, 
some accept LP tokens,
and others accept more than one ERC20 token.

In \ref{item:phase2}, some protocols focus on lending strategies, others on leveraged borrowing or liquidity provision strategies. Some protocols employ multiple strategy groups.


* Fully diluted market cap: theoretical market cap which is calculated by assuming all the tokens were already in circulating supply.
\label{tab:overview}
\vspace{-6mm}
\end{table*}



==> exhibits/empirical_plots.tex <==

\begin{figure*}[ht]
\centering
    % \subfloat[Total pool shares\label{fig:total_supply_vault}]
    %     {\includegraphics[height=0.15\textheight,width=0.33\textwidth]{figures/vault_DAI_total_supply.pdf}
    %     \includegraphics[height=0.15\textheight,width=0.33\textwidth]{figures/vault_USDC_total_supply.pdf}
    %     \includegraphics[height=0.15\textheight,width=0.33\textwidth]{figures/vault_3crv_total_supply.pdf}}
    
    % \subfloat[Price per share\label{fig:price_per_share}]
    %     {\includegraphics[height=0.15\textheight,width=0.33\textwidth]{figures/vault_DAI_price_per_share.pdf}
    %     \includegraphics[height=0.15\textheight,width=0.33\textwidth]{figures/vault_USDC_price_per_share.pdf}
    %     \includegraphics[height=0.15\textheight,width=0.33\textwidth]{figures/vault_3crv_price_per_share.pdf}}

\caption{Empirical data}
\label{fig:empirical_results}
\end{figure*}

==> exhibits/mechanism_phase2.tex <==
\begin{figure}
\centering
% \includegraphics[width = \linewidth]{figures/mechanism_workflow-Phase2}
\caption{Execution process of a single strategy. SC = Smart Contract}
\label{fig:mechanism_phase2}
\end{figure}


==> exhibits/mechanism_worklfow.tex <==
\begin{figure}[h!]
\centering
% \includegraphics[width=\linewidth]{figures/mechanism_workflow_v2-All.pdf}
\caption{Stylized yield aggregator mechanism}
\label{fig:mechanism_all}
\end{figure}



==> exhibits/notation.tex <==
\begin{table}
\caption{Mathematical notations for Idle Finance models}
\begin{tabularx}{8.4cm}{lX}
\toprule
Notation & Definition     \\     \midrule
$n$                 &   the number of lending protocols used          \\
$x_i$               &   the amount (in underlying) allocated in protocol $i$       \\
$nextRate(x_i)$     &   a function which returns the new APR for protocol $i$ after supplying $x_i$         \\
$nextScore(x_i)$    &   a function which returns the new Score for protocol $i$ after supplying $x_i$ amount of underlying         \\
$maxnextRate$       &   the highest rate of all implemented protocols after supplying $x_i$ amount         \\
$maxnextScore$      &   the highest score of all implemented protocols after supplying $x_i$ amount         \\
$k$                 &   a coefficient for expressing weights of score and APR         \\
$tot$               &   the total amount to rebalance  \\
\bottomrule
\end{tabularx}
\label{tab:idleFinanceNotation}
\end{table}

==> exhibits/strategies_cases.tex <==
\begin{figure}[tbp]
\centering
% \subfloat[Simple lending\label{fig:simpleLending}]
%     {\includegraphics[width=0.5\textwidth]{figures/mechanism_workflow_v2-strat_case_1.pdf}}\hfill
% \subfloat[Leveraged borrow\label{fig:leveragelending}]
%     {\includegraphics[width=0.5\textwidth]{figures/mechanism_workflow_v2-strat_case_3}}\hfill
% \subfloat[Liquidity provision\label{fig:liqmining}]
%     {\includegraphics[width=0.5\textwidth]{figures/mechanism_workflow-strat_case_2}}
\caption{Classic yield aggregator strategies}
\label{fig:example_strategies}
\end{figure}

==> exhibits/top_yield.tex <==
\newpage
\begin{landscape}
\begin{table*}[t]
  \centering
  \caption{}
  \tiny
  \begin{adjustbox}{width=\textwidth}
  \begin{tabularx}{\linewidth}{lXccccccccccccc}
    Yield aggregators & Simple lending & Leveraged borrow & Liquidity provision & TVL(m USD) & year established & Market cap(m USD) & Chains & Governance token & Token holders \\
    \midrule
    Convex Finance & \Circle & \Circle & \CIRCLE & 3,649.50 & May 2021 & 513.36 & Ethereum & CVX & 13,604 \\
    Arrakis Finance & \Circle & \Circle & \CIRCLE & 1830  & Feb 2021 &       & Ethereum, Polygon, Optimism & SPICE &  \\
    Alpaca Finance & \Circle & \CIRCLE & \Circle & 533.3 & Jul 2021 & 38.19 & BNB, Fantom & ALPACA & 1,501 \\
    Aura  & \CIRCLE & \Circle & \Circle & 273.16 & Jul 2021 & 25.8  & Ethereum & AURA & 482 \\
    Coinwind & \Circle & \Circle & \Circle & 224.4 & Jul 2022 &       & BNB, Ethereum, Heco & COW & 80 \\
    Tulip Protocol & \Circle & \CIRCLE & \Circle & 163.39 & May 2021 & 5.24  & Solana & TULIP & 787 \\
    Quarry & \Circle & \Circle & \Circle & 140.86 & Nov 2021 &       & Solana &       &  \\
    Sunny & \Circle & \Circle & \CIRCLE & 119.83 & Aug 2021 & 1.21  & Solana & SUNNY & 302 \\
    Vector Finance & \Circle & \Circle & \CIRCLE & 106.83 & Mar 2022 & 2.98  & Avalanche & VTX & 3 \\
    Concentrator & \Circle & \Circle & \CIRCLE & 102.96 & Mar 2022 &       & Ethereum & CTR & 112 \\
    StakeDAO & \CIRCLE & \Circle & \Circle & 102.69 & Mar 2021 & 25.21 & Ethereum, Polygon, Avalanche, Harmony, BSC & SDT & 3,959 \\
    Tranchess & \CIRCLE & \CIRCLE & \CIRCLE & 102.42 & Jun 2021 & 32.16 & BNB   & CHESS & 1,041 \\
    Tokemak & \Circle & \Circle & \CIRCLE & 85.35 & Jul 2021 & 29.7  & Ethereum & TOKE & 5,129 \\
    Francium & \CIRCLE & \CIRCLE & \Circle & 77.22 & Oct 2021 &       & Solana &       &  \\
    Homora & \CIRCLE & \CIRCLE & \CIRCLE & 65.65 & Oct 2020 & 57.95 & Ethereum, Avalanche, BSC, Fantom & ALPHA & 8,958 \\
    Bunny & \CIRCLE & \Circle & \Circle & 62.67 & Apr 2021 & 0.049 & BNB, Polygon & BUNNY & 18,705 \\
    Dot Dot Finance & \Circle & \Circle & \CIRCLE & 44    & Apr 2022 &       & BNB   & DDD &  \\
    Belt Finance & \Circle & \Circle & \CIRCLE & 42.65 & May 2021 & 1.86  & BNB, Heco, Klaytn & BELT &  \\
    Liquid Driver & \CIRCLE & \CIRCLE & \Circle & 31.89 & Jun 2021 & 5.27  & Fantom & LQDR &  \\
    Element Finance & \CIRCLE & \Circle & \CIRCLE & 31.39 & Oct 2021 &       & Ethereum &       &  \\
    \end{tabularx}%
  \label{tab:addlabel}%
  \end{adjustbox}
\end{table*}%
\end{landscape}

==> exhibits/yield_assets.tex <==
\begin{figure}[ht]
\centering
% \includegraphics[width=55mm,scale=0.5]{figures/yield_assets.pdf}
\caption{Yield sources and representative crypto assets associated with each source. \coin{cTokens} and \coin{aTokens} are interest-bearing tokens from the lending markets Compound and Aave respectively. Uniswap and Sushiswap LP tokens are tied to their respective AMMs. \coin{COMP}, \coin{UNI} and \coin{CRV} are governance tokens that have been or are currently being distributed to protocol users of Compound, Uniswap and Curve, respectively, as part of the liquidity mining program. \coin{VSP} and \coin{SUSHI} are governance tokens of Vesper and Sushiswap distributed in a liquidity mining program, as well as tokens entitled to revenue sharing when they are staked within their protocol.}
\label{fig:yield_assets}
\end{figure}



==> sections/comparison.tex <==

\section{Current Major yield aggregators in DeFi}
\label{sec:comparison}

To date, yield aggregators have collected billions of dollars worth of liquidity. \autoref{fig:tvl} charts the evolution of total value locked for current major protocols since July 2020. This number indicates the total amount of funds that users deposited in different yield aggregators on Ethereum. 
This section compares current major yield aggregator protocols with a focus on strategies, performance and fee mechanism.

\autoref{tab:overview} shows the characteristics of the current major protocols and a few more. The data was collected on 19 December 2021. 
% The fully diluted market cap for Yearn finance reaches 1,520.8 million USD and the number of \coin{YFI} token holders is 40,089, achieving the largest market dominance of 0.07\% amongst all the protocols. TVL of Yearn finance amounts to 4,787.7 million USD, followed by Harvest Finance with 481.1 million USD.



\subsection{Idle Finance}

Launched in August 2019, Idle is a yield aggregator that automatically allocates and aggregates interest-bearing tokens \cite{idle2021documentation}. 

% \subsubsection{Pools}

% At the time of writing\footnote{\label{noteToday}\today}, the following pools are available in Idle Finance, depending on the strategy:
% \begin{itemize}
%     \item Best-Yield: {\tt DAI}, {\tt USDC}, {\tt USDT}, {\tt SUSD}, {\tt TUSD}, {\tt WETH}, {\tt WBTC}
%     \item Risk-Adjusted: {\tt DAI}, {\tt USDC}, {\tt USDT}
% \end{itemize}


\subsubsection{Strategies}

Idle Finance only distributes single-asset pools over different lending protocols.
In \ref{item:phase0}, users' funds are pooled together and depending on the strategy that the pool employs, assets are allocated over different lending platforms, currently\footnote{\label{noteToday}\today} limited to: Compound, Fulcrum, Aave, DyDx and Maker DSR. There is no need for \ref{item:phase1} in Idle Finance, as the currently supported pools can be deposited directly into the above lending platforms. When any user interacts with Idle or if no interactions are made for 1 hour, rebalancing of the assets takes place according to the rates of supported providers.
% The result is that the underlying position of {\tt IdleTokens} holders is dynamically rebalanced . Depending on the strategy, the act of rebalancing is modeled differently. 

Currently, Idle uses two different allocation strategies:
\begin{itemize}
    \item Best-Yield: this strategy seeks the best interest rates across multiple lending protocols.
    \item Risk-Adjusted: this strategy automatically changes the asset pool allocation in order to find an allocation with the highest risk-return score, compared to the highest return score of the \enquote{Best Yield} strategy. It does this by incorporating a framework for quantifying risk, developed by DeFiScore \cite{defiscore2021}, which outputs a 0-10 score that represents the level of risk on a specific lending platform (0 = highest risk, 10 = lowest risk).
\end{itemize}


\subsubsection{Return for users}

Idle uses {\tt IdleTokens} to represent the farmers' proportional ownership of the asset pool, which should accrue yield over time. In addition, farmers are rewarded with \coin{IDLE} governance tokens for participating in the pools as part of Idle's liquidity mining program. In January 2021, a two-year liquidity mining program started to reward liquidity providers depending on the amount of funds deposited and the utility generated by a certain pool \cite{idle2021distribution}.


\subsubsection{Protocol fees}

A performance fee 10\% of the generated yield is charged.
%, calculated by subtracting the current {\tt IdleToken} price (expressed in the underlying asset) by the average {\tt IdleToken} price at the moment of minting and multiplying this by 0.1. The price in USD is defined by the amount of yield that has been collected since its inception and the price of the underlying token (in USD). 
% The collected fees flow to a treasury contract that is governed by the {\tt IDLE} governance token holders.


%----------------------------------------------------------------

\subsection{Pickle Finance}

Launched in September 2020, Pickle offers yield on deposits through two products: Pickle Jars (pJar) and Pickle Farms. Jars are yield farming robots, earning returns on users' funds, while farms are liquidity mining pools where users can earn {\tt PICKLE} governance tokens by staking different kinds of assets. Proportional shares in pJars are represented by \coin{pTokens}.

% \subsubsection{Pools}

% A total of 19 different Pickle Jars are currently deployed, where the necessary funds to be supplied are LP tokens from Uniswap, Sushiswap or Curve. Besides those Jars, 12 Pickle Farms are active, where users either provide their {\tt pTokens} or {\tt UNI PICKLE-ETH} LP tokens. 

\subsubsection{Strategies}

Each Pickle Jar employs a specific strategy to earn yield. Currently, two main versions of pJar strategy are in existence, pJar 0.00 and pJar 0.99, of which the 0.99 version is most important. There is no \ref{item:phase1} involvement in either version, pooled funds are directly utilized to farm rewards in \ref{item:phase2}, after which they are sold in \ref{item:phase3} to re-invest the accrued yield.

\begin{itemize}
    \item pJar 0.00: These pJars involve a user depositing LP tokens acquired by supplying liquidity on Curve Finance \cite{Curve2021}, an AMM-based DEX (see \ref{sec:amm}). The strategy employed in pJar 0.00 earns and re-invests \coin{CRV} rewards by selling \coin{CRV} into the market for stablecoins and re-depositing those into the Curve pools to get more LP tokens. Effectively, pJars 0.00 generate yield by accruing
    \begin{enumerate*}[label={(\roman*)}]
    \item LP fees from Curve and
    \item generating \coin{CRV} tokens because of Curve's liquidity mining program \cite{curve2021tokenomics}.
    \end{enumerate*}
    \item pJar 0.99: These pJars utilize LP tokens from Uniswap and Sushiswap, earning yield by accruing
    \begin{enumerate*}[label={(\roman*)}]
    \item LP fees from Uniswap/ Sushiswap and 
    \item generating \coin{SUSHI} or other native tokens because of liquidity mining programs.
    \end{enumerate*}
\end{itemize}


\subsubsection{Return for users}

Return of Pickle users is generally composed of
    \begin{enumerate*}[label={(\roman*)}]
    \item the fees accrued by providing liquidity to AMM pools,
    \item earning tokens distributed through external liquidity mining programs, and
    \item extra \coin{PICKLE} tokens if the yield farmer makes use of the Farm products. 
    \end{enumerate*}
    The return is thus dependent on underlying market forces, liquidity programs and token values. For example, the Pickle emission schedule defines how much \coin{PICKLE} will be distributed over time \cite{pickle2021emission}. 

% Because many of the Pickle Jars strategies require depositing LP tokens, returns will further be impacted by the value change of LP tokens themselves---commonly denominated in \coin{ETH} or fiat-pegged stablecoin---due to market trading activities (see Section~\ref{subsec:examples}).
% Because Curve pools only contain equal-pegged stablecoins, Curve LP jars (pJar 0.00) are less prone to this particular kind of loss. 

\subsubsection{Protocol fees}

Most Pickle Jars have a 20\% performance fee on the generated yield.
% , except for the Sushi pJars and two others. 
% Those fees are collected by the Pickle Treasury contract. 


%-----------------------------------------------------------

\subsection{Harvest Finance}

Harvest Finance gives \coin{FARM} holders the opportunity to share in the revenue model of the protocol. By staking \coin{FARM}, users are entitled to receive part of the revenue that is collected by the protocol. Harvest Finance went live in August 2020, and currently has more than 
70 pools/vaults in its offering. 

% \subsubsection{Pools}

% Funds are supplied into Harvest Vaults, which are divided in different categories. At the time of writing, there are 13 stablecoin-related vaults, 5 Sushi HODL vaults, one ETH2.0 vault, 5 \coin{BTC}-related vaults, 5 NFT-related vaults, 6 Sushiswap vaults, 5 Uniswap Liquidity vaults, 4 seigniorage vaults, 6 mSTONKs vault, 1 \coin{LINK} vault and 2 main vaults including a \coin{WETH} and profit-sharing \coin{FARM} vault.

\subsubsection{Strategies}

Harvest Finance has two main categories of yield farming strategies~\cite{harvest2021strategies}:

\begin{itemize}
    \item Simple single-asset Strategies: Users deposit single assets such as \coin{USDC}, \coin{USDT}, \coin{DAI}, \coin{WBTC}, \coin{renBTC} or \coin{WETH} into a Harvest Vault, which then deposits those assets into another yield generating protocol, including Compound and Idle Finance. 
    \item LP token Strategies: Users deposit LP tokens from Uniswap, Sushiswap or Curve into Harvest which automatically collects liquidity mining rewards and re-invests them into LP tokens.
\end{itemize}



\subsubsection{Return for users}

Depending on the vault used, return of Harvest users is composed of
\begin{enumerate*}[label={(\roman*)}]
\item the fees accrued by providing liquidity to AMM pools or other yield-bearing assets, 
\item earning tokens distributed through external liquidity mining programs and 
\item extra \coin{FARM} tokens as part of the liquidity mining program. 
\end{enumerate*}
These returns are dependent on underlying market forces, liquidity programs and token values. For example, the Harvest emission schedule defines how much \coin{FARM} will be distributed over time \cite{harvest2021token}.

% Similar to Pickle Finance, as many of the Harvest strategies require depositing LP tokens, the ever-changing value of LP tokens also affects returns. 
% , divergence loss should be smaller for Curve LP token strategy pools.

\subsubsection{Protocol fees}

Harvest Finance does not charge withdrawal fees and does not claim a direct ``fee'' on the yield farming revenue. However, during liquidation of the yield, 30\% of the profits is used to buy the \coin{FARM} token on the market, which is then distributed to users who stake \coin{FARM} in the profit-sharing \coin{FARM} pool \cite{harvest2021vaultFunction}.\footnote{This type of buyback reduces the supply of governance tokens in the secondary market to the benefit of existing tokenholders.}


%-----------------------------------------------------------

\subsection{Yearn Finance}
\label{subsec:yearn}

Yearn Finance offers a multitude of products in Decentralized Finance (DeFi), providing lending aggregation, yield generation and others \cite{yearn2021intro}. The services discussed here are Yearn Earn, a lending aggregator, and Yearn Vaults, a more comprehensive yield aggregator. Yearn Finance launched in July 2020.




% \subsubsection{Pools}

% Both Earn pools and Vaults have a number of possible deposit assets. 
% Earn pools: There are seven separate Earn pools at the time of writing. Users can deposit \coin{DAI}, \coin{USDC}, \coin{USDT}, \coin{TUSD}, \coin{SUSD}, \coin{WBTC} and \coin{BUSD}. There are a total of 50 Vaults, of which 36 are v1 Vaults and 14 are v2 Vaults. Vaults are either single-asset or Curve LP tokens. There are currently no Vaults for Uniswap-like LP tokens.

\subsubsection{Strategies}

\begin{itemize}
    \item Earn pools: The strategy of the Earn pools is to collect a certain asset and deposit it either in dYdX, Aave or Compound, depending on where the highest interest rate of that asset is found. Yearn will withdraw from one protocol and deposit to another automatically as interest rates change between protocols. Earn pools thus omit \ref{item:phase1} and go directly to \ref{item:phase2}, in a strategy that is slightly similar to the Idle Finance ``Best-Yield'' Strategy. Proportional shares in Earn pools are commonly represented by \coin{yTokens}.
    \item Vaults: A Yearn Vault uses an asset as liquidity, deposits that liquidity as collateral (accounting for risk levels) to borrow stablecoins. Then, it uses those stablecoins to generate yield, after which that yield is re-invested in the stablecoins to generate more yield. Vaults thus employ all phases as illustrated in \autoref{fig:mechanism_all}, and allows for more complex strategies compared to Earn pools. Proportional shares in Yearn Vaults are commonly represented by \coin{yvTokens} or other \coin{yTokens}.
    
    % v1 Vaults \cite{yearn2021v1} are created and maintained by a Controller, who oversees the strategy execution. When the original funds are used to open a collateralized debt position, the collateralization ratio is always monitored to avoid being liquidated. 
    
    % v2 Vaults improved the capital efficiency of v1 Vaults by including 4 main improvements. One v2 Vault can have up to 20 strategies, increasing the flexibility during different market scenarios. Second, the Controller in v1 Vaults is replaced by a Strategist and a Guardian. Third, some of the smart contract functions are automated through the use of Keep3r bots \cite{cronje2021keepr}, unloading humans from these housekeeping tasks. The fourth improvement concerns testing upgrades. A simplified visualization can be seen on \cite{vasa2021viz}. 
\end{itemize}

Yield farming strategies (\ref{item:phase2}) in Yearn v2 Vaults can be complex, involving flash loans (uncollateralized loans that are taken and repaid within the same transaction \cite{Xu2021c}), leveraged borrowing, staking on specific protocols (for example HegicStaking) and more. 


\subsubsection{Return for users}

Yearn Finance distributed the \coin{YFI} governance token over a 9-day period after launch. Liquidity providers in the Earn pools or Vaults are thus not incentivized by a Yearn liquidity mining program, so current yield only comes from the returns that the product strategies reap. Those returns can be straightforward, as is the case for Earn pools, and can be complex to calculate, as is the case for v2 Vaults that can have up to 20 strategies working at once. Some Yearn vaults accept LP tokens, other accept single asset tokens.

\subsubsection{Protocol fees}

v1 Vaults have a 20\% performance fee and a 0.5\% withdrawal fee (in case funds need to be pulled from the strategy in order to cover the withdrawal request). v2 Vaults have also a 20\% performance fee, but no withdrawal fee. Instead, they charge a 2\% management fee. Performance fees are split 50:50 between the Treasury and the Strategist, the official creator of the strategy. The management fee is assigned fully to the Treasury.

% EARN POOLS FEE??



\subsection{Empirical performance}

By fetching on-chain data of the above mentioned four main protocols, we visualized the evolution of selected vaults for comparison purposes. The evolution of a) total supply, and b) price per share are plotted for the \coin{DAI} vault, \coin{USDC} vault, and \coin{3crv} vault for aggregators where these specific pools are available. \coin{3crv} is the LP token name for the \href{https://curve.fi/3pool}{Curve Finance 3pool}. The name ``vaultTokens'' is used to represent the share of the corresponding Token-pool in a specific protocol. The price per share represents the ratio of underlying tokens and vaultTokens, which should be 1-to-1 pegged to a certain currency in the beginning.

Generally, the value of the vaultTokens then increases relatively compared to the underlying token as yield is accrued and added to the pool. Results are obtained by collecting the block where the vault is created, and calling the respective view functions with a block interval of 500 blocks until August 2021. The obtained timelines are shown in \autoref{fig:empirical_results}.

Regarding the total pool supply, Yearn shows an overall increase till June 2021 for all vaults, while those of the other protocols are either stable or volatile (especially in vault3crv).
Meanwhile, the surge in total supply for Harvest vaultUSDC in the middle of October 2020, followed by the drop at the end of the same month coincides with the surge in TVL of Harvest by 21st October (TVL achieved 704.1 million USD on 21st October, up 110\% from 334.41 million USD a week earlier), and the Harvest flash loan attack on 26th October, respectively.
In the attack, an attacker stole funds from the \coin{USDC} and \coin{USDT} vaults of Harvest Finance. A malicious actor had exploited an arbitrage and temporary loss, allowing this actor to obtain vault shares for a beneficial price, after which they were burned for profit \cite{HarvestFinance2020}. Looking at the vault3crv, drops in total supply of Harvest Finance are observed at the beginning of January 2021 and towards the end of February 2021 as well.

Concerning price per share, the number steadily increases overall, aside from the sharp declines observed for Harvest vaultDAI and vaultUSDC at the end of October 2020. These are again attributed to the flash loan attack that occurred on 26th October, where funds were drained out of the pool without equally affecting the number of vaultDAI. Further, the graph shows that the Yearn vaults update their contract relatively often, resulting in a short lifespan of plots---otherwise, a sharp decrease in price per share might have been observed after the attack against Yearn Finance on 4 February 2021, in which an unknown entity stole 2.8 million USD, resulting in Yearn's \coin{DAI} vault losing 11.1 million USD \cite{yearn2021exploit}.
The hacker(s) exploited the vault using Aave---a complex exploit with over 160 nested transactions and 8.6 million gas used (around 75\% of the block) reportedly resulted in a loss of 2.7 million USD \cite{Etherscan}.
% , tweeted by Stani Kulechov, the founder of DeFi platform Aave. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Other aggregators}

The four main yield aggregators above are deemed the most mature, but a new wave of yield aggregating protocols is coming up. In general, there seems to be a tendency where more recent yield aggregators aim to be a one-stop-shop, providing additional functionalities such decentralized exchanges, lending and borrowing and risk-managing services. This enhances user experience and introduces more revenue streams for the protocols.

Below we list more recently launched protocols and products that are still being tested.

\paragraph{Vesper Finance}
Vesper \cite{vesper2021} 
% introduces themselves as ``a DeFi ecosystem and growth engine for crypto assets", by providing ``a suite of yield-generating products, focused on accessibility, optimization, and longevity". The company 
focuses on institutional adoption of the DeFi yield market. Currently, only Vesper Grow Pools are available, which are comparable to the traditional yield products. In future developments, Vesper plans to integrate 
% Vesper Earn, Vesper Stake and Vesper Labs , which will allow the user to be exposed to yield in many ways. 
Vesper Labs \cite{vesper2021} where external users can build their own strategy in return for part of the reaped profits. 
% Although this seems promising from a flexibility perspective, it will be interesting to see how safe these strategies will be considered. 
% As described in Table~\ref{tab:overview}, fully diluted market cap for Vesper finance is 337.0 million USD and the VSP token holders are 5,387. The market dominance is 0.00\%. TVL amounts to 1,468.7 million USD and the price is 33.7 USD, as of 1st May.


\paragraph{Rari Capital}
Rari Capital \cite{rari2021} is a roboadvisor that attempts to provide investors with the highest yield, beyond just lending. It has multiple products, including Earn, Tranches, Fuse and Tanks. The Earn product can be considered a traditional yield farming service, while the other products are extending the number of functionalities on the Rari Capital platform, such as lending and borrowing, and yield farming within certain risk boundaries, called ``tranches'' \cite{rariTranches2020}.
% The fully diluted market cap amounts to 173.0 million USD, while the RGT token holders are 9,319, achieving the market dominance of 0.01\%. TVL is as much as 90.1 million USD and the price is 17.3 USD, as of 1st May.

\paragraph{Value DeFi}
Value DeFi \cite{valuedefi2021} has developed three main products: Value Liquid, Farming services and Vaults. Value liquid is an AMM platform, with vSwap and vPegSwap, allowing users to trade assets and earn fees if they provide liquidity in pools. The farming services, called vFarms, offer users staking possibilities with different returns. The vaults, called vSafes, are the more standard yield-generating contracts as discussed in this paper. 


\paragraph{Alpha Homora}
Alpha Homora provides leveraged yield farming and leveraged liquidity provision. Users can participate in various roles in Alpha Homora, including Yield Farmers, Liquidity Providers, \coin{ETH} Lenders, Liquidators, and Bounty Hunters \cite{alpha2021docs}. This protocol does not specifically focus on extending the number of functionalities in one application, but more on allowing users to leverage their positions.

\paragraph{Bank of Chain}
Bank of Chain (BoC) offers automated yield farming services for stablecoins on EVM-compatible blockchains including Ethereum, Polygon and BNB Chain. 
The protocol  
supports widely-adopted USD-pegged stablecoins such as \coin{DAI}, \coin{USDC} and \coin{USDT}. The BoC vault collects stablecoin deposits which are consequently invested in a range of pre-selected yield-generating pools from other vetted protocols. Fund deployment, yield farming, reinvestment of yield, portfolio re-balancing are all automatically conducted following a pre-programmed strategy.


\subsection{Summary}

Many yield farming strategies entail some extent of optimization, e.g. choosing the lending pool that offers the highest APY to deposit assets into (e.g. Idle's Best-Yield pools, Yearn's earn pools), or balancing between risks and return (e.g. Idle's risk-adjusted pools). The core strategies applied by major yield aggregators commonly do not deviate much from the basic strategies described in \autoref{sec:formalization}. However, as the competition in yield farming grows, basic strategies becomes less effective \cite{Jakub}, which prompts protocols to device more sophisticated strategies that incorporate various forms of interactions with other DeFi protocols (e.g. upgrade from Yearn v1 to v2). Yield aggregators generate revenues by charging fees from investors. Protocols associated with better yield farming performance are able to charge higher fees, which can be observed by comparing both the performance fee between Yearn (20\%) and Idle (10\%) as well as their respective performance (see \autoref{fig:price_per_share}).



% the relationship between the problem yield aggregators are trying to solve, i.e., the optimization problems they target, and challenges elsewhere in finance or computer science? In other words, why is it hard to build such a system and what existing principles can designers draw on



